The Stackage Repository: An Exploratory Study of its Evolution

Context. Package repositories for a programming language are increasingly common. A repository can keep a register of the evolution of its packages. In the programming language Haskell, with its defining characteristic monads, we can find the Stackage repository, which is a curated repository for stable Haskell packages in the Hackage repository. Despite the widespread use of Stackage in its industrial target, we are not aware of much empirical research about how this repository has evolved, including the use of monads. Objective. This paper conducts empirical research about the evolution of Stackage considering monad packages through 22 Long-Term Support releases during the period 2014-2023. Focusing on five research questions, this evolution is analyzed in terms of packages with their dependencies and imports; including the most used monad packages. To the best of our knowledge, this is the first large-scale analysis of the evolution of the Stackage repository regarding packages used and monads. Method. We define six research questions regarding the repository's evolution, and analyze them on 51,716 packages (17.05 GB) spread over 22 releases. For each package, we parse its cabal file and source code to extract the data, which is analyzed in terms of dependencies and imports using Pandas scripts. Results. From the methodology we get different findings. For example, there are packages that depend on other packages whose versions are not available in a particular release of Stackage; opening a potential stability issue. The mtl and transformers are on the top 10 packages most used/imported across releases of the Stackage evolution. We discussed these findings with Stackage maintainers, which allowed us to refine the research questions.

==> free-flags.tex <==
\resizebox{\columnwidth}{!}{
\begin{tabular}{c | l}%p{1.7in}}
\textbf{Flag} & \textbf{\free Monads used} \\
\toprule
Alternative & \co{Control.Alternative.Free}, \co{Control.Alternative.Free.Final} \\

Applicative &  \co{Control.Applicative.Free}, \co{Control.Applicative.Free.Fast}, \co{Control.Applicative.Free.Final} \\

A.Trans & \co{Control.Applicative.Trans.Free} \\

Comonad & \co{Control.Comonad.Cofree}, \co{Control.Comonad.Cofree.Class}, \co{Control.Comonad.Trans.Cofree}, \co{Control.Comonad.Coiter} \\

Free & \co{Control.Monad.Free}, \co{Control.Monad.Free.Ap}, \co{Control.Monad.Free.Church}, \co{Control.Monad.Free.Class}, \co{Control.Monad.Free.TH} \\

M.Trans & \co{Control.Monad.Trans.Free}, \co{Control.Monad.Trans.Free.Ap}, \co{Control.Monad.Trans.Free.Church}, \co{Control.Monad.Trans.Iter} \\

\bottomrule
\end{tabular}
}

==> logger-flags.tex <==
%\resizebox{\columnwidth}{!}{
\begin{tabular}{c | l}%p{1.7in}}
\textbf{Flag} & \textbf{\monadlogger Monad used} \\
\toprule
Logger & \co{Control.Monad.Logger} \\
\bottomrule
\end{tabular}
%}

==> mtl-flags.tex <==
\resizebox{\columnwidth}{!}{
\begin{tabular}{c | l}%p{1.7in}}
\textbf{Flag} & \textbf{\mtl Monads used} \\
\toprule
Cont & \co{Control.Monad.Cont}, \co{Control.monad.Cont.Class} \\

Error &  \co{Control.Monad.Error}, \co{Control.Monad.Error.Class} \\

Identity & \co{Control.Monad.Identity} \\

List & \co{Control.Monad.List} \\

RWS & \co{Control.Monad.RWS}, \co{Control.Monad.RWS.Class}, \co{Control.Monad.RWS.Lazy}, \co{Control.Monad.RWS.Strict} \\

Reader & \co{Control.Monad.Reader}, \co{Control.Monad.Reader.Class} \\

Writer & \co{Control.Monad.Writer}, \co{Control.Monad.Writer.Class}, \co{Control.Monad.Writer.Lazy}, \co{Control.Monad.Writer.Strict} \\

State & \co{Control.Monad.State}, \co{Control.Monad.State.Class}, \co{Control.Monad.State.Lazy},  \co{Control.Monad.State.Strict} \\

Trans & \co{Control.Monad.Trans}, \co{Control.Monad.Trans.Class} \\

Except & \co{Control.Monad.Except} (available only since version 2.2.1) \\
\bottomrule
\end{tabular}
}

==> results.tex <==
% !TEX root = main.tex

\section{Results: Answering RQs}
\label{sec:results}

This section answers the five research questions presented at the beginning of this paper. Each answer is accompanied by a graph or table at least. 

%%%%
\subsection{Regarding RQ1}
\label{sec:rq1}

Figure~\ref{fig:depencyEvolution} shows a dependency network graph for three releases of \stackage: first, middle, and the last one in 2020. At a first glance, we can clearly observe that the number of dependencies increases with the number of new packages in the repository. During the \stackage evolution, we can observe that the top 8 packages keep their dependency ranks: \co{time}, \co{mtl}, \co{transformer}, \co{text}, \co{containers}, \co{bytestring}, \co{filepath}, and \co{vector}. Although the \mtl package is not the most used (in terms of dependencies), we can mention this package has been widely used in the evolution of the repository. Finally, this figure shows that categories of the top packages are varied.

According to versions of dependencies per package, we present two findings. First, \fref{fig:rq1_2} shows the number and percentage of packages whose dependency versions are not available in its \stackage release, meaning that are non-stable dependencies for that release. Although these packages are few, there is a growing trend that might affect the stability promise of \stackage. Second, \fref{fig:rq1_3} shows that some packages depend on the same package but with different ranges of versions; making incompatible dependencies of packages. %The packages with incompatible dependencies are not necessarily the same per release,                  

%the top 15 packages that are the most used in \stackage. Of the fourteen releases analyzed, the top 5 packages are commonly \co{base}, \co{bytestring}, \co{containers}, \co{text}, and \co{transformers}. As the table also shows, the \mtl package is the sixth most used, meaning that monads are widely used. The top 22 most used package is \co{quickchek}, a package for testing and this does not appear in the table for space reasons. This package is outside of the \stackage selection, compromising the stability promise given by this repository. In the next question, we analyze the {\em outside packages} issue in detail. 


%Table~\ref{tbl:releases} shows the top 15 packages that are the most used in \stackage. Of the fourteen releases analyzed, the top 5 packages are commonly \co{base}, \co{bytestring}, \co{containers}, \co{text}, and \co{transformers}. As the table also shows, the \mtl package is the sixth most used, meaning that monads are widely used. The top 22 most used package is \co{quickchek}, a package for testing and this does not appear in the table for space reasons. This package is outside of the \stackage selection, compromising the stability promise given by this repository. In the next question, we analyze the {\em outside packages} issue in detail. 


\subsection{Regarding RQ2}
\label{sec:rq2}

To answer this question we use Figures~\ref{fig:rq2_1} and~\ref{fig:rq2_2}, which show two box graphs that answer the average of dependencies that are direct and indirect respectively. 

Figure~\ref{fig:rq2_1} shows that the number of direct dependencies is less than 10 and is almost constant around the \stackage evolution. Few packages are outside of this average, where the outlier number of direct dependencies is around 90. Instead, Figure~\ref{fig:rq2_2} shows that the number of indirect dependencies is higher and its variance is also higher. Regarding indirect dependencies, many packages can be considered outliers, showing that the average (less than 10) of these dependencies is not so representative.      

%Figure~\ref{fig:rq2} shows the number and percentage of packages that are outside of the \stackage selection. We can see in this figure that for the first release, 12\% of packages are (in)directly outside of \stackage. In next releases, this percentage increases to 17\%, implying a potential stability issue that is not being addressed in this repository so far. Some of these packages are \co{quickcheck}, \co{microlens}, \co{hunit}, and \co{cabal}. This last package is currently deprecated, but there are still dependencies that depend on this deprecated version. The use of a deprecated dependency to manage \co{.Cabal} files may affect to a repository system that use these files to be structured.      

\subsection{Regarding RQ3}
\label{sec:rq3}

The first release contains only 800 packages and then many packages have been added to \stackage in the following releases. Figure~\ref{fig:rq3} shows how often these packages are updated between releases. Whereas we can see a higher percentage of packages are updated between releases 2-22 and 6-35, there is also a smaller number of updates between releases 12-14 and 13-19. An explanation for this finding is the interval of time between releases. In the beginning there is an average of 6 months per release, then there is only an average of 3 months per release. 
%In the last release analyzed (16-11), we found 5,069 of 16,611 dependencies specify \co{any} in its version required, meaning that use the last version available in the \stackage release.       


\subsection{Regarding RQ4}
\label{sec:rq4}

Figure~\ref{fig:rq4} shows the use of different monads in \stackage. In the figure, we can see that the \co{State} and \co{Reader} monads have a strong presence against to other monads. This presence may be due to both monads allow developers to express stateful pieces of code. In addition, the figure shows that the uses of \co{Error} and \co{Exception} are inversely proportional, possibly due to \co{Exception} is able to work as a replacement for \co{Error} in various scenarios. In fact, \co{Exception} increases its presence while \co{Error} decreases in each release.         



\subsection{Regarding RQ5}
\label{sec:rq5}

As this research question is composed of two subquestions, we used two graphs to answer. Figure~\ref{fig:rq5a} shows the packages added and removed from releases that import \mtl modules. First releases add a higher amount of packages than the last releases; indeed, the last releases remove more packages than added. Between releases 7-24 and 11-24, we can see a considerable fluctuation of packages that are added and removed. As a big picture, this figure shows that from the release 11-22, more packages that import \mtl are removed than added. On the contrary, Figure~\ref{fig:rq5b} shows the number of packages that start and stop using \mtl modules. The first finding is that few packages add/remove the use of \mtl over time (approximately 3 packages per release). We explained this result because of the strong need for monads to implement certain operations (\eg mutable states).    

\bigskip

\parhead{Summary} We can observe the top 8 most used packages, including \mtl, remain constant. In addition, the use of \mtl in added packages has apparently decreased over time. As downside points, we can highlight two ones. First, a growing trend of packages {\em a)} are depending on other packages whose versions are not available in a particular release and {\em b}) have incompatible version dependencies with other packages; opening a potential stability issue. Second, \stackage presents unstructured fields for metadata such as {\em category} and {\em stability}, which is an issue that comes from the \hackage repository because \stackage uses its metadata.      


\endinput


==> transformers-flags.tex <==
\resizebox{\columnwidth}{!}{
\begin{tabular}{c | l}%p{1.7in}}
\textbf{Flag} & \textbf{\transformers Monads used} \\
\toprule
Applicative & \co{Control.Applicative.Backwards}, \co{Control.Applicative.Lift} \\

Signatures &  \co{Control.Monad.Signature} \\

Trans & \co{Control.Trans.Accum}, \co{Control.Trans.Class}, \co{Control.Trans.Cont}, \co{Control.Trans.Except}, \co{Control.Trans.Identity}, \co{Control.Trans.Maybe} \\

RWS & \co{Control.Monad.Trans.RWS}, \co{Control.Monad.Trans.RWS.CSP}, \co{Control.Monad.Trans.RWS.Lazy}, \co{Control.Monad.Trans.RWS.Strict} \\

Reader & \co{Control.Monad.Trans.Reader} \\

Select & \co{Control.Monad.Trans.Select} \\

State & \co{Control.Monad.Trans.State}, \co{Control.Monad.Trans.State.Lazy}, \co{Control.Monad.Trans.State.Strict} \\

Writer & \co{Control.Monad.Trans.Writer}, \co{Control.Monad.Trans.Writer.CPS},  \co{Control.Monad.Trans.Writer.Lazy},  \co{Control.Monad.Trans.Writer.Strict} \\

\bottomrule
\end{tabular}
}
